Learning of Causal Observable Functions for Koopman-DFL Lifting Linearization of Nonlinear Controlled Systems and Its Application to Excavation Automation

Effective and causal observable functions for low-order lifting linearization of nonlinear controlled systems are learned from data by using neural networks. While Koopman operator theory allows us to represent a nonlinear system as a linear system in an infinite-dimensional space of observables, exact linearization is guaranteed only for autonomous systems with no input, and finding effective observable functions for approximation with a low-order linear system remains an open question. Dual-Faceted Linearization uses a set of effective observables for low-order lifting linearization, but the method requires knowledge of the physical structure of the nonlinear system. Here, a data-driven method is presented for generating a set of nonlinear observable functions that can accurately approximate a nonlinear control system to a low-order linear control system. A caveat in using data of measured variables as observables is that the measured variables may contain input to the system, which incurs a causality contradiction when lifting the system, i.e. taking derivatives of the observables. The current work presents a method for eliminating such anti-causal components of the observables and lifting the system using only causal observables. The method is applied to excavation automation, a complex nonlinear dynamical system, to obtain a low-order lifted linear model for control design.

==> algo-cont.tex <==
\section{Modeling Algorithm}
\label{sec:algo}
% In this paper, we seek to apply the modeling benefits of DFL to learned latent spaces. Note that the finite-dimensional matrix representation of the Koopman operator $\mathcal{K}$ is related to the coefficient matrix $H$ in DFL. Because Koopman operators were originally only applied to autonomous systems, the domain of $\mathcal{K}_fg$ is $\mathbb{R}^m$. Because DFL models nonautonomous systems and uses $\eta$ to augment, rather than replace, the state, the domain of $H$ is larger, $\mathbb{R}^{l+m+n}$, enabling a higher-dimensional linear parametrization of the dynamics. By treating all parameters of the DFL model, $g$, $A$, and $H$, as learnable, we can avoid the modeling pitfalls of previous works, enabling a data-driven, time- and state-independent, lifted linearization algorithm capable of directly tracking the system state without dictating a control algorithm.

% Because we treat $A$ as a learnable parameter, in addition to minimizing the residual term, $r_\eta(x_t,u_t)$, we must override the state transition function from DFL in Eq. \ref{eq:dfl-x-dyn} to include a residual term as well:
% \begin{equation}
%     x_{t+1}=A_x x_t+A_\eta \eta_t+B_x u_t+r_x(x_t,u_t)
%     \label{eq:dfl-x-dyn-res}
% \end{equation}

% By redefining the goal of the modeling problem purely to minimize the dual residual of the augmented linear model, data-driven state augmentation should produce more exact results than traditional DFL and previous work on machine learning for linear latent spaces.

% \subsection{Learning Framework}

Fig. \ref{fig:blocks} shows the overview of the modeling algorithm. First we assume all state variables are accessible and sufficient data for training are attainable. All state variables are fed into the left neural network, $g(x)$, to produce a set of synthetic observables $\eta_t$ to be learned. The state $x_t$, observables $\eta_t$, and input $u_t$ are fed into the Linear Dynamic Model with parameter matrices $A$ and $H$. The linear model produces predicted state $\hat{x}_{t+1}$ and predicted observables $\hat{\eta}_{t+1}$. The predicted state $\hat{x}_{t+1}$ is compared to the true value $x_{t+1}$, while the predicted observables are compared to their ground truth $\eta_{t+1}$ that is produced by the same neural network in response to the state $x_{t+1}$. The second neural network in the figure is a twin copy of the first neural network, sharing the same weights in it.

The squared error of the predicted state and observables, $J$, is used for updating the Linear Dynamic Model with respect to parameters $A$ and $H$ and the neural network weights. The update of these parameters is computed via Error Back Propagation (EBP).

The causality analysis involved in the DFL modeling allows us to examine whether  observables, called auxiliary variables, are functions of state alone, or include inputs. If some auxiliary variables are causal, having no dependence on control input, they can be added to the state for lifting the dynamics. Let $\zeta*_t$ be causal auxiliary variables. As shown in Fig. \ref{fig:blocks}, the causal observables can be fed into the neural network, so that the synthetic auxiliary variables $\eta_t$ can be produced from richer data. Note that the ground truth $\eta_{t+1}$, too, can be produced in response to not only state $x_{t+1}$ but also $\zeta_{t+1}$. The tunable parameter space of the neural network is expanded with the use of the causal auxiliary variables.

In case physically measurable auxiliary variables are functions of both state and input, such input-dependent auxiliary variables cannot be used in their original form for lifting the dynamics. It is necessary to filter out the input components from the observables. Fig. \ref{fig:blocks} also shows a simple filter to eliminate the effect of input from those variables, $\zeta_t$, as discussed in Sec. \ref{sec:algo}.

In this section, we will first describe the continuous-time learned lifting linearization, then modify the model where necessary for discrete-time implementation. Finally, we will extend the theory for anticausal observables.

In this section, we will first describe the continuous-time learned lifting linearization, then modify the model where necessary for discrete-time implementation. Finally, we will extend the theory for anticausal observables.

\subsection{Continuous-Time Learned Lifting Linearization}
Consider a continuous-time dynamic system given by:
\begin{equation}
    \dot x(t)=f(x(t),u(t))
\end{equation}

Let $g$ be a randomly initialized neural network encoder model to generate the synthetic observables, $\eta$:
\begin{equation}
    \eta(t;\theta)=g(x(t);\theta)
    \label{eq:eta-defn}
\end{equation}

Define a datum vector $\xi(t;\theta)\triangleq \left( x^\intercal(t), \eta^\intercal(t;\theta), u^\intercal(t) \right)^\intercal$. Let $A\in \mathbb{R}^{l\times p}$ and $H\in \mathbb{R}^{m\times p}$ be randomly initialized matrix coefficients modeling the state and augmented state transition dynamics, respectively. We override Eq. \ref{eq:cases-dfl} to include residuals in the original and augmented state vectors:
\begin{equation}
    \begin{cases}
        \dot x(t)=A\xi(t)+r_{\dot x(t)} \\
        \dot \eta(t)=H\xi(t)+r_{\dot \eta(t)} \\
        \eta(0)=g(x(0))
    \end{cases}
    \label{eq:cases-dfl-res}
\end{equation}

Given observation data of $\dot x$, $x$, and $u$ as $\dot x_{\mathrm{ob}}$, $x_{\mathrm{ob}}$, and $u_{\mathrm{ob}}$, respectively, we synthesize observations of the augmented state,
\begin{equation}
    \eta_{\mathrm{ob}}=g(x_{\mathrm{ob}})
\end{equation}
and its derivative,
\begin{equation}
    \dot \eta_{\mathrm{ob}}=\frac{d\eta_{\mathrm{ob}}}{dt}=\frac{d\eta_{\mathrm{ob}}}{dx_{\mathrm{ob}}} \frac{dx_{\mathrm{ob}}}{dt}=\left. g'\right|_{x_{\mathrm{ob}}}\dot x_{\mathrm{ob}}
\end{equation}
and assemble a datum vector $\xi_{\mathrm{ob}}\triangleq \left( x_{\mathrm{ob}}^\intercal, \eta_{\mathrm{ob}}^\intercal, u_{\mathrm{ob}}^\intercal \right)^\intercal$ for each observation.

For each observation, we can compute associated residuals by rearranging Eq. \ref{eq:cases-dfl-res}:
\begin{equation}
    \begin{cases}
        r_{\dot    x_\mathrm{ob}}=\dot    x_{\mathrm{ob}}-A\xi_{\mathrm{ob}} \\
        r_{\dot \eta_\mathrm{ob}}=\dot \eta_{\mathrm{ob}}-H\xi_{\mathrm{ob}}
    \end{cases}
\end{equation}

We define a quadratic loss function, $J_\mathrm{ob}$, used to train the model:
\begin{equation}
    J_\mathrm{ob}\triangleq r_{\mathrm{ob}}^\intercal Qr_{\mathrm{ob}}
    \label{eq:cost}
\end{equation}
where $Q$ is a matrix coefficient and $r_{\mathrm{ob}}$ is a total residual given by
\begin{equation}
    r_{\mathrm{ob}} \triangleq \left( r_{\dot x_\mathrm{ob}}^\intercal, r_{\dot \eta_\mathrm{ob}}^\intercal \right)^\intercal
    \label{eq:exp-tot-res}
\end{equation}

Model parameter matrices $A$ and $H$, as well as the parameters of the neural network, $\theta$, are computed by solving the following optimization problem:
\begin{equation}
    \theta^o, A^o, H^o=\argmin_{\theta,A,H}\mathrm{E} \left[ J_\mathrm{ob}(\theta,A,H) \right]
    \label{eq:grad-desc}
\end{equation}

There are two approaches to obtaining the optimal parameters $\theta^o$, $A^o$, and $H^o$. One is based on least squares estimation combined with a gradient-based method, and the other is solely based on gradient-based optimization.
\subsubsection{Least Squares Estimate}
Eq. \ref{eq:grad-desc} can be reduced to:
\begin{equation}
    \begin{array}{rl}
        \theta^o, A^o, H^o & =\argmin_\theta \left[ \min_{A,H} \left[ \mathrm{E} \left[ J_\mathrm{ob}(\theta,A,H) \right] \right] \right] \\
        & =\argmin_\theta \mathrm{E} \left[ J_\mathrm{ob}(\theta;A^o(\theta),H^o(\theta)) \right]
    \end{array}
\end{equation}
where $A^o(\theta)$ and $H^o(\theta)$ are the optimal coefficient matrices that minimize the squared error for a given parameter of the neural net, $\theta$. For $Q=I$:
\begin{equation}
    \begin{cases}
        A^o(\theta)=\mathrm{E}\left[ x_t \xi_{t-1}^\intercal(\theta) \right]\left( \mathrm{E} \left[ \xi_{t-1}(\theta)\xi_{t-1}^\intercal(\theta) \right] \right)^{-1} \\
        H^o(\theta)=\mathrm{E}\left[ g(x_t;\theta) \xi_{t-1}^\intercal(\theta) \right]\left( \mathrm{E} \left[ \xi_{t-1}(\theta)\xi_{t-1}^\intercal(\theta) \right] \right)^{-1}
    \end{cases}
    \label{eq:opt-a-h}
\end{equation}

The optimization of the neural network parameter, $\theta$, can be performed by using an error backpropagation algorithm. The cost functional $J_\mathrm{ob}\left( \theta;A^o(\theta),H^o(\theta) \right)$, however, is highly complex; the partial derivatives of this cost functional with respect to $\theta$ are complex and computationally expensive. Although $J_\mathrm{ob}\left( \theta;A^o(\theta),H^o(\theta) \right)$ has been optimized in terms of $A$ and $H$, the overall computation may be more complex.

\subsubsection{Gradient-Based Approach}
An alternative is to treat the linear dynamic model as another layer of the neural network and apply the error backpropagation algorithm through the extended network. Since the evolution of state, $x$, and synthetic observables, $\eta$ is linear, both can be represented with a single layer of the network with a linear activation function. Fig. XXX shows the network structure. The linear dynamic model is the output layer of the augmented neural network. The $\delta$-values associated with the final layer units can be computed directly from the squared error:
\begin{equation}
    \begin{cases}
        \delta_{x_i}=-\frac{\partial J_\mathrm{ob}}{\partial x_i}\quad i=1,\ldots,l \\
        \delta_{\eta_j}=-\frac{\partial J_\mathrm{ob}}{\partial \eta_j}\quad j=1,\ldots,m
    \end{cases}
\end{equation}
where the activation function is linear with unity slope. Simply backpropagating these $\delta$-values, the parameters of the neural network, $\theta$, can be trained.

The least squares estimate approach entails a centralized process with a large batch size for computing $A^o(\theta)$ and $H^o(\theta)$ in Eq. \ref{eq:opt-a-h}. In contrast, in the gradient-based approach, no batch processing is required, as mini-batch processing will be sufficient.

% Model parameters of $g$, $A$, and $H$ are computed by solving the following optimization problem:
% \begin{equation}
%     \hat g, \hat A, \hat H = \argmin_{g,A,H}\mathrm{E} \left[ J_\mathrm{ob} \right]
%     \label{eq:grad-desc}
% \end{equation}

% We solve the problem in Eq. \ref{eq:grad-desc} using gradient-based optimization. For a parameter, $\theta$,
% \begin{equation}
%     \mathrm{grad}_\theta \mathrm{E}\left[ J_\mathrm{ob} \right]=\mathrm{E} \left[ 
%     r_\mathrm{ob}^\intercal \left(Q^\intercal +Q\right)\frac{\partial r_\mathrm{ob}}{\partial \theta}
%     \right]
%     \label{eq:grad-theta}
% \end{equation}

% Consider a scalar parameter at row $i$, column $j$ of $A$, $a_{i,j}$. Its residual gradient from Eq. \ref{eq:grad-theta} can be computed as
% \begin{equation}
%     \frac{\partial r_\mathrm{ob}}{\partial a_{i,j}}=o_i^{l+m}\xi_{\mathrm{ob},j}
% \end{equation}
% where $o_i^p$ is a one-hot vector of length $p$ of which the $i^{\mathrm{th}}$ element is 1 and $\xi_{\mathrm{ob},j}$ is the $j^\mathrm{th}$ element of $\xi_\mathrm{ob}$.

% Likewise, consider a scalar parameter at row $i$, column $j$ of $H$, $h_{i,j}$. Its residual gradient can be computed as
% \begin{equation}
%     \frac{\partial r_\mathrm{ob}}{\partial h_{i,j}}=o_{l+i}^{l+m}\xi_{\mathrm{ob},j}
% \end{equation}

% Finally, consider a scalar parameter of neural network $g$, $\theta_g$. Its residual gradient can be computed as
% \begin{equation}
%      \frac{\partial r_\mathrm{ob}}{\partial \theta_g}=\left( \begin{array}{c}
%           -\left. A_\eta\frac{\partial g}{\partial \theta_g} \right|_{x_\mathrm{ob}} \\
%           \left. \frac{\partial^2 g}{\partial \theta_g \partial x} \right|_{x_\mathrm{ob}}\dot x_\mathrm{ob} - H_\eta\left. \frac{\partial g}{\partial \theta_g} \right|_{x_\mathrm{ob}}
%           \end{array} \right)
%           \label{eq:grad-g-cont}
% \end{equation}
% where the derivatives are computed via backpropagation.

\subsection{Discrete-Time Learned Lifting Linearization}
Let $x_t$ and $u_t$ be the state and control input, respectively, of the discrete-time dynamic system given by Eq. \ref{eq:disc-dyn-nonaut} at time $t$. Let $g$ be a randomly initialized neural network encoder model to generate the augmented state, $\eta_t=g(x_t)$. Let $\xi_t\triangleq \left( x_t^\intercal, \eta_t^\intercal, u_t^\intercal \right)^\intercal$. As before, we approximate the system dynamics using the DFL equation
\begin{equation}
    \begin{cases}
        x_{t+1}=A\xi_t+r_{x_{t+1}} \\
        \eta_{t+1}=H\xi_t+r_{\eta_{t+1}}
    \end{cases}
    \label{eq:dfl-simplified-x-disc}
\end{equation}
where $A$ and $H$ are randomly initialized matrix coefficients and $r_x(x_t,u_t)$ and $r_\eta(x_t,u_t)$ are residual terms to account for nonlinearities not captured in $\eta_t$.

The residual minimization problem in discrete time is simpler than in continuous time. By applying the discrete-time shift operator $T_{-1}$ to the above equations, we can avoid taking derivatives altogether and rewrite the discrete-time residuals:
\begin{equation}
    \begin{cases}
        r_{x_t}=x_t-A\xi_{t-1} \\
        r_{\eta_t}=\eta_t-H\xi_{t-1}
    \end{cases}
\end{equation}

Given observations at consecutive times, we again tune $g$, $A$, and $H$ using Eq. \ref{eq:grad-desc}. The absence of $\dot \eta_\mathrm{ob}$ allows us to simplify Eq. \ref{eq:grad-g-cont}:
\begin{equation}
    \frac{\partial}{\partial \theta_g}\left( \begin{array}{c}
        r_{x_t} \\
        r_{\eta_t}
    \end{array} \right) = \left( \begin{array}{c}
        -A_\eta\left. \frac{\partial g}{\partial \theta_g} \right|_{x_{t-1}} \\
        \left. \frac{\partial g}{\partial \theta_g} \right|_{x_t}-H_\eta \left. \frac{\partial g}{\partial \theta_g} \right|_{x_{t-1}}
    \end{array} \right)
\end{equation}

We repeat the above steps with each new batch of data.

\subsection{Extension to Anticausal Observables}
As discussed in \cite{asada-dfl}, augmenting the state with physical observables is often useful. Because this learned lifting linearization is data-driven, augmenting the state, $x$, with control-independent, physical observables is trivial. However, as reviewed in Sec. \ref{sec:bkgnd}, if the augmented state is dependent on the control input, the augmented system dynamics may become anticausal. Consider a vector of physical observables, $\zeta(x,u)$, suspected of including a dependence on $u$. As in \cite{korda2018linear,asada-dfl}, and \cite{mamakoukas2019local}, assume that this dependence is linear:
\begin{equation}
    \zeta(x,u)=\zeta^*(x)+Du
    \label{eq:zeta}
\end{equation}
where $\zeta^*(x)$ is exclusively a function of state and $D$ is a fixed matrix coefficient of $u$. Because $\zeta^*(x)$ is uncorrelated with the control input, $\mathrm{E}\left[ \zeta^*(x) u^\intercal \right] =0$. Therefore, multiplying Eq. \ref{eq:zeta} by $u^\intercal$ and taking the expectation yields:
\begin{equation}
    \mathrm{E}\left[ \zeta(x,u)u^\intercal \right]=D\mathrm{E}\left[ uu^\intercal \right]
\end{equation}

Given observations of $\zeta(x,u)$ and $u$, computing $D$ becomes a least-squares linear regression:
\begin{equation}
    \hat D=\mathrm{E}\left[ \zeta(x,u)u^\intercal \right]\mathrm{E}\left[ uu^\intercal \right]^{-1}
\end{equation}

Before training the learned lifted linearization model in Eq. \ref{eq:dfl-simplified-x-disc}, we preprocess the data to ``clean'' the physical observables from any linear dependence on $u$ via
\begin{equation}
    \zeta^*(x_{\mathrm{ob}})=\zeta(x_{\mathrm{ob}},u_{\mathrm{ob}})-\hat Du_{\mathrm{ob}}
    \label{eq:clean-zeta}
\end{equation}
for each observation.

Then, we augment the DFL model to include $\zeta^*(x)$. We override Eq. \ref{eq:eta-defn}:
\begin{equation}
    \eta(t)=g\left( \left( \zeta^{*\intercal}(x(t)), x^\intercal(t) \right)^\intercal \right)
    \label{eq:eta-defn-zeta}
\end{equation}
and follow the same training procedure described above to tune $g$, $A$, and $H$ using Eq. \ref{eq:grad-desc}.
